Towards a Flow- and Path-Sensitive Information Flow Analysis: Technical Report

This paper investigates a flow- and path-sensitive static information flow analysis. Compared with security type systems with fixed labels, it has been shown that flow-sensitive type systems accept more secure programs. We show that an information flow analysis with fixed labels can be both flow- and path-sensitive. The novel analysis has two major components: 1) a general-purpose program transformation that removes false dataflow dependencies in a program that confuse a fixed-label type system, and 2) a fixed-label type system that allows security types to depend on path conditions. We formally prove that the proposed analysis enforces a rigorous security property: noninterference. Moreover, we show that the analysis is strictly more precise than a classic flow-sensitive type system, and it allows sound control of information flow in the presence of mutable variables without resorting to run-time mechanisms.

==> transform-example.tex <==
\lstset{numbers=left}
%\newsavebox\TransformationOriginal
%\begin{lrbox}{\TransformationOriginal}
%\begin{minipage}{0.2\textwidth}
%\begin{lstlisting}
%$x := \high$; 
%$x := 0;$ 
%$\low := x$;
%$y := x + 1;$
%if $\low$ < 0 then $y := \high$; 
%if $\low$ > 0 then $x := y$; 
%while ($x>\low$)
%	x = x + 1;
%\end{lstlisting}
%\end{minipage}
%\end{lrbox}
\newsavebox\TransformationBracket
\begin{lrbox}{\TransformationBracket}
\begin{minipage}{0.2\textwidth}
\begin{lstlisting}
$x := \high$; 
$\bkassign{x}{0};$ 
$\low := x$;
$y := x + 1;$
if ($x$ = 0) then 
	$\bkassign{y}{\high}$; 
if ($x$ > 0) then 
	$\assign{\low}{y}$; 
while ($x<10$)
	$\bkassign{x}{x+1}$;
\end{lstlisting}
\end{minipage}
\end{lrbox}
\newsavebox\TransformationTransformed
\begin{lrbox}{\TransformationTransformed}
\begin{minipage}{0.2\textwidth}
\begin{lstlisting}
$x :=\high$; 
$x_1 := 0;$ 
$\low := x_1$;
$y := x_1 + 1;$
if $x_1$ = 0 then {
	$y_1 := \high$;  
	$y_2 := y_1$	}
else 
	$y_2 := y$;
if ($x_1$ > 0) then 
	$\low := y_2$;
$x_2 := x_1$;
while ($x_2<10$) {
	$x_3 := x_2 + 1$; 
	$x_2 := x_3$ }
\end{lstlisting}
\end{minipage}
\end{lrbox}
\begin{figure}
	\centering
%	\subfigure[Original Program]{
%		\label{fig:example:transform:original}\
%		\usebox\TransformationOriginal
%	}
%	\quad
	%
	\subfigure[Source Program]{
		\label{fig:example:transform:bracket}\
		\usebox\TransformationBracket
	}
	%
	\subfigure[Transformed Program]{
		\label{fig:example:transform:transformed}\
		\usebox\TransformationTransformed
	}
	\caption{Examples illustrating program transformation}
	\label{fig:example:transformation}
%	\vspace{-0.05in}
\end{figure}

==> transform-semantics.tex <==
\begin{figure}
	\begin{align*}
	&\text{Vars}       &x, y, z ∈\; &\Varst \\
	&\text{Expr} \quad &\et::=\; &x \mid n \mid \et~\op~\et \\
	&\text{Cmds} \quad &\cmdt  ::=\; &\Skip \mid \cmdt_1;\cmdt_2 \mid \assigneta{x}{\et} \mid \while{\cmdt}{\et} \\ %\phiassigneta{\actset_1(\overrightarrow{X})}{\actset_2(\overrightarrow{X})} \mid  \\
	&                  &            &\ifcmd{\et}{\cmdt_1}{\cmdt_2}  \\
%		&                  &            & \repeatconteta{\cmdt}{\et}
	\end{align*}
	\caption{Syntax of Transformed Language}
	\label{fig:transform-syntax}
\end{figure}



\begin{figure*}
\begin{mathpar}
	\inferrule{ }{\configTwo{\Mt}{n} \evalto {n}} 
	\and 
	\inferrule{ }{\configTwo{\Mt}{x} \evalto {\Mt(x)}}
	\and
	\inferrule{\configTwo{\Mt}{\et_1} \evalto {n_1}
				\quad \configTwo{\Mt}{\et_2} \evalto {n_2}
				\quad n = n_1\ \op\ n_2	}
	{
		\configTwo{\Mt}{\et_1\ \op\ \et_2} \evalto {n}}
\end{mathpar}
\begin{mathpar}
\inferrule[ST-Skip]
{ }{\configTwo{\Mt}{\Skip;\cmdt} \To \configTwo{\Mt}{\cmdt}}
\and
\inferrule[ST-Seq]
{\configTwo{\Mt}{\cmdt_1} \To \configTwo{\Mt'}{\cmdt_1'} }
{\configTwo{\Mt}{\cmdt_1; \cmdt_2} \To \configTwo{\Mt'}{\cmdt_1';\cmdt_2}}
\and
\inferrule[ST-While]
{ }
{ \configTwo{\Mt}{\while{\cmdt}{\et}} \To \configTwo{\Mt}{\ifcmd{\et}{(\cmdt;\while{\cmdt}{\et})}{\Skip}} }
\and
\inferrule[ST-Assign]
{\configTwo{\Mt}{\et} \evalto {n} }
{\configTwo{\Mt}{\assigneta{x}{\et}} \To \configTwo{\Mt\Mupdate{x}{n}}{\Skip} }
\and
\inferrule[ST-If1]
{\configTwo{\Mt}{\et} \evalto n \quad n \neq 0  }
{\configTwo{\Mt}{\ifcmd{\et}{\cmdt_1}{\cmdt_2}} \To \configTwo{\Mt}{\cmdt_1}	}
\and
\inferrule[ST-If2]
{\configTwo{\Mt}{\et} \evalto n \quad n = 0  }
{\configTwo{\Mt}{\ifcmd{\et}{\cmdt_1}{\cmdt_2}} \To \configTwo{\Mt}{\cmdt_1}	}
\and
%\inferrule[ST-Phi]
%{ \overrightarrow{X_1} = \actset_1(\overrightarrow{X})
%	\quad \configTwo{\Mt}{\actset_2(\overrightarrow{X})} \evalto \overrightarrow{V}   }
%{\configTwo{\Mt}{\phiassigneta{\actset_1(\overrightarrow{X})}{\actset_2(\overrightarrow{X})}} \To \configTwo{\Mt\Mupdate{\overrightarrow{X_1}}{\overrightarrow{V}}}{\Skip} }
%\and
%\and
%\inferrule[ST-Cont]
%{ }
%{ \configTwo{\Mt}{\repeatconteta{\cmdt}{\et}} \To \configTwo{\Mt}{\cmdt;\ifcmd{\et}{\Skip}{(\repeatuntil{\cmdt}{\et})}} }
\end{mathpar}
\caption{Transformed Program Semantics}
\label{fig:transform-semantics}     
\end{figure*}



